Early Discovery of Emerging Entities in Microblogs

Keeping up to date on emerging entities that appear every day is indispensable for various applications, such as social-trend analysis and marketing research. Previous studies have attempted to detect unseen entities that are not registered in a particular knowledge base as emerging entities and consequently find non-emerging entities since the absence of entities in knowledge bases does not guarantee their emergence. We therefore introduce a novel task of discovering truly emerging entities when they have just been introduced to the public through microblogs and propose an effective method based on time-sensitive distant supervision, which exploits distinctive early-stage contexts of emerging entities. Experimental results with a large-scale Twitter archive show that the proposed method achieves 83.2% precision of the top 500 discovered emerging entities, which outperforms baselines based on unseen entity recognition with burst detection. Besides notable emerging entities, our method can discover massive long-tail and homographic emerging entities. An evaluation of relative recall shows that the method detects 80.4% emerging entities newly registered in Wikipedia; 92.4% of them are discovered earlier than their registration in Wikipedia, and the average lead-time is more than one year (571 days).

==> sandbox.tex <==
\begin{table*}[t]
\scriptsize
    \centering
        \caption{The statistics of the emerging entities and their contexts obtained from our Twitter archive by distant supervision.}\label{table:ds}
        \begin{tabular}{llrr|l@{\ }l}
            \toprule
            \textbf{TYPE} & \textbf{DBpedia types} & \textbf{\# entities} & \textbf{\# examples} & \multicolumn{2}{l}{\textbf{examples of emerging context (translated)}} \\ 
            \midrule
PERSON
& Actor & 885 & 2863 & * & Expected new rookie voice actor ``\textbf{Sora Amamiya}'' appeared for the first time on \\ 
& MusicalArtist & 731 & 4616 & &  live broadcasting! It is becoming a topic to be...  \\
& SoccerPlayer & 531 & 2327 & * & I saw Koibumi X and it's very good. \textbf{Riho Yoshioka} and \textbf{Ayano Kaneko} will \\
& VoiceActor & 484 & 1596 & &  be famous in the future, I think.  \\
& BaseballPlayer & 419 & 4390 & *&  We won the right to negotiate Mr. \textbf{Masashi Kato} of JR East Tohoku with \\
%& AdultActor & 299 & 1731 & &   nomination of  6th  draft.\\
%& Model & 281 & 1343 & * & Ms. \textbf{Daruma Matsuura}, who won the prize when I reviewed the newcomer award, \\
%& Politician & 260 & 1164 & & seems to start serializing from the next number. \\
%& Person & 177 & 729 & * & In Kawasaki Mayor's election, Mr. \textbf{Norihiko Fukuda} defeated the nomination  \\
%& Writer & 152 & 542 & &  candidate and was elected for the first time.\\
%& Wrestler & 136 & 576 & * & You'd better follow the youngster, \textbf{Atsugiri Jason}, who has been working for 2 \\ 
%& ComicsCreator & 93 & 361 & &   months since joining OHTA PRODUCTION. \\
%& Presenter & 80 & 370 & * & Defeat 19th place in the world in the tour debut game! The world is paying \\
%& FigureSkater & 74 & 165 & &  attention to \textbf{Naomi Osaka}.\\
%& AthleticsPlayer & 68 & 296 & * & Yokohama DeNA Baystars announces that it has agreed to sign a player  contract for\\
%& BasketballPlayer & 66 & 175 & &  the 2017 season with \textbf{Spencer Patton}. \\
%& MilitaryPerson & 48 & 110 & * & I saw ``Saints - End of Promise -'' at the New Theater in Yokohama. It is a debut  \\
%& Comedian & 36 & 182 & & work of  featured director \textbf{David Rowley} !!! \\
%& ComedyGroup & 28 & 82 & * & Mika, who is the partner of me has changed her name from ``Mika Tabura'' to \\
%& VolleyballPlayer & 21 & 70 & & ``\textbf{Momo Nonotomiya}''.  \\
%& Scientist & 19 & 94 & * & Nice to meet you, I am \textbf{Tamotsu Kansyuji} from the Juno-Super-Boy Contest. \\
%& TennisPlayer & 15 & 67 & & From now  on I will try my best as an actor. Thank you.  \\
%& Artist & 14 & 43\\
& (\# entities $< 15$) & 29 & 90\\
\midrule
& Sub Total & 4932 & 23939\\
\midrule
CREATIVE WORK
& MusicSingle & 1321 & 11685 & * & I started an official account. It was announced at a Shonen Jump  released today, a \\
& TelevisionShow & 1153 & 8478& &  new series ``\textbf{My Hero Accademia}'' starts from next week! \\
& MusicAlbum & 970 & 6092 & * & Marvel \& Sony officially announced that the title of the rebooted version \\
& Film & 917 & 6307 & &  Spider-Man is \textbf{Spider-Man: Homecoming }. The logo was also released. \\
& VideoGame & 652 & 6355 & * & Congratulations on ``\textbf{Re: Zero-Starting Life in Another World}'' for upcoming \\
& Manga & 623 & 2561 & & publication ! \\
%& Anime & 323 & 2983 & * & Please give us a message at reply as we will record the first broadcast to \\
%& RadioProgram & 266 & 1010 & &  commemorate \textbf{Sasara Night of Fujioka Minami} on the STV radio.   \\
%& Book & 146 & 983 & * & [Digest News] Asratec enters the robot software business with control software \\
%& Song & 32 & 174 & &     called ``\textbf{V-Sido OS}'' \\
%& Software & 28 & 360 & * & KADOKAWA and Hatena's novel posting site ``\textbf{Kakuyomu}'' will open on February \\
%& Website & 23 & 188 & &   29,  2016. Web novel contest will be also held. \\
& (\# entities $< 15$) & 6 & 91 & \\
\midrule
& Sub Total & 6460 & 47267 \\
\midrule
LOCATION
& Building & 121 & 756 & * & As the result of voting, the name of the station to be constructed at the JR Nambu \\
& Museum & 42 & 184 & &  branch line is decided as \textbf{Odaei Station}!  \\
& Station & 34 & 115 & * & \textbf{Kumagai Morikazu Tsukechi Museum of Art} opening ceremony commenced. \\
%& Settlement & 28 & 47 & &  Director Konan's greetings are taking place.  \\
%& School & 24 & 34 & * & A new gourmet building ``\textbf{Ueno no Mori Cherry Terrace}'' is born in Ueno. Both \\
%& City & 17 & 46 & &  lunch and dinner can be eaten there. \\
%& University & 14 & 47 & *\\
%& Mountain & 14 & 44 & \textcolor{white}{*}\\
%& Park & 11 & 30 & *\\
& (\# entities $< 15$) & 102 & 372 & \\
\midrule
& Sub Total & 371 & 1554 \\
\midrule
GROUP
& Company & 259 & 1441 & * & With the entry of robot business, Softbank established the new company \textbf{Cocoro} \\
& Organisation & 28 & 179 & &  \textbf{SB} today on June 5. \\
& PoliticalParty & 24 & 249 & * &  Mr. Ishiba decided on Friday to set up a faction and name it ``\textbf{Suigetsukai}.''\\
\midrule
& Sub Total & 311 & 1869 \\
\midrule
OTHER
& Species & 77 & 337 & * & New species \textbf{Sado flog}, found on Sado Island, features yellow feet and belly.\\
%& CelestialBody & 17 & 75 & * & Although it is the first discovered asteroid ``\textbf{2014 AA},'' it is likely that it collided \\
& (\# entities $< 15$) & 19 & 38 & &  with the Earth and apparently burned out in the atmosphere. \\
%& owl:Thing & 14 & 102\\
%& others & & \\
\midrule
& Sub Total & 116 & 459 \\
\midrule
UNMAPPED && 7417 & 35958 & * & Rival of Airplay? New Wi-Fi standard ``\textbf{Miracast}'' transmit video wirelessly.\\
&&&& * & Production of the chip \textbf{Apple A9} for the next iPhone has been started. \\
& &&& * & JMA named the heavy rain ``\textbf{Heavy Rainfall in Kanto / Tohoku H27.9}''.\\
         \midrule
			\textbf{Total} && 19604 & 111046\\
			\bottomrule
        \end{tabular}

\end{table*}

\begin{table}[t]
\scriptsize
    \centering
        \caption{Relative recall and time advantage over entity types of emerging entities detected by \textbf{Proposed (LSTM-CRF)}.}
        \begin{tabular}{llrr@{\quad}rrrr@{\quad}r}
            \toprule
             \multicolumn{2}{l}{\textbf{TYPE}} & \textbf{\# entities} & \multicolumn{2}{r}{\textbf{\# found (\%)}} & \multicolumn{4}{r}{\textbf{lead-days}} \\ 
            & \textbf{DBpedia types} & & & & \multicolumn{4}{r}{\textbf{mean (median)}} \\ 
            \midrule

\multicolumn{2}{l}{PERSON} &&&&\\	
& Actor & 651 & 506 & (77.73\%) & & & 753 & (750)\\
& MusicalArtist & 624 & 457 & (73.24\%) & & & 749 & (659)\\
& SoccerPlayer & 477 & 427 & (89.52\%) & & & 775 & (762)\\
& VoiceActor & 345 & 317 & (91.88\%) & & & 508 & (376)\\
& AdultActor & 306 & 300 & (98.04\%) & & & 376 & (297)\\
%& BaseballPlayer & 238 & 213 & (89.50\%) & & & 591 & (405)\\
%& Model & 225 & 210 & (93.33\%) & & & 764 & (654)\\
%& Person & 173 & 136 & (78.61\%) & & & 788 & (804)\\
%& Politician & 136 & 112 & (82.35\%) & & & 665 & (538)\\
%& Wrestler & 116 & 97 & (83.62\%) & & & 360 & (165)\\
%& Presenter & 86 & 77 & (89.53\%) & & & 635 & (552)\\
%& Writer & 83 & 65 & (78.31\%) & & & 504 & (376)\\
%& AthleticsPlayer & 72 & 66 & (91.67\%) & & & 918 & (927)\\
%& ComicsCreator & 63 & 50 & (79.37\%) & & & 853 & (753)\\
%& BasketballPlayer & 50 & 35 & (70.00\%) & & & 759 & (701)\\
%& Comedian & 48 & 37 & (77.08\%) & & & 665 & (424)\\
%& ComedyGroup & 44 & 31 & (70.45\%) & & & 681 & (643)\\
%& FigureSkater & 40 & 22 & (55.00\%) & & & 797 & (809)\\
%& MilitaryPerson & 32 & 22 & (68.75\%) & & & 312 & (173)\\
%& Artist & 15 & 9 & (60.00\%) & & & 772 & (718)\\
%& VolleyballPlayer & 14 & 13 & (92.86\%) & & & 811 & (918)\\
%& TennisPlayer & 6 & 3 & (50.00\%) & & & 1033 & (1456)\\
%& Scientist & 3 & 2 & (66.67\%) & & & 1591 & (1591)\\
%& Photographer & 2 & 2 & (100.00\%) & & & 691 & (691)\\
%& MartialArtist & 1 & 1 & (100.00\%) & & & -104 & (-104)\\
%& FictionalCharacter & 1 & 1 & (100.00\%) & & & 951 & (951)\\
& (\# entities $< 15$) & 42 & 31 & (73.81\%) & & & 838 & (918)\\
\midrule
& Sub Total & 3851 & 3211 & (83.38\%) & & & 665 & (556)\\
\midrule
\multicolumn{2}{l}{CREATIVE WORK}&&&&\\	
& TelevisionShow & 699 & 640 & (91.56\%) & & & 228 & (55)\\
& MusicSingle & 653 & 593 & (90.81\%) & & & 305 & (85)\\
& Film & 641 & 552 & (86.12\%) & & & 391 & (214)\\
& MusicAlbum & 550 & 498 & (90.55\%) & & & 356 & (161)\\
& Manga & 523 & 481 & (91.97\%) & & & 678 & (600)\\
%& VideoGame & 440 & 391 & (88.86\%) & & & 407 & (249)\\
%& RadioProgram & 228 & 203 & (89.04\%) & & & 261 & (38)\\
%& Anime & 216 & 184 & (85.19\%) & & & 261 & (91)\\
%& Book & 101 & 94 & (93.07\%) & & & 627 & (463)\\
%& Website & 24 & 16 & (66.67\%) & & & 869 & (624)\\
%& Song & 23 & 21 & (91.30\%) & & & 549 & (301)\\
%& Software & 22 & 9 & (40.91\%) & & & 817 & (723)\\
%& Artwork & 2 & 1 & (50.00\%) & & & 160 & (160)\\
& (\# entities $< 15$) & 2 & 1 & (50.00\%) & & & 159 & (159)\\
\midrule
& Sub Total & 4122 & 3683 & (89.35\%) & & & 379 & (179)\\
\midrule
\multicolumn{2}{l}{LOCATION}&&&&\\	
& Building & 89 & 73 & (82.02\%) & & & 505 & (291)\\
& Museum & 33 & 32 & (96.97\%) & & & 685 & (447)\\
%& Station & 25 & 21 & (84.00\%) & & & 264 & (154)\\
%& School & 18 & 9 & (50.00\%) & & & 554 & (74)\\
%& Library & 13 & 13 & (100.00\%) & & & 995 & (1328)\\
%& Park & 11 & 9 & (81.82\%) & & & 639 & (193)\\
%& University & 7 & 6 & (85.71\%) & & & 904 & (996)\\
%& Temple & 7 & 4 & (57.14\%) & & & 1457 & (1446)\\
%& Shrine & 6 & 3 & (50.00\%) & & & 528 & (304)\\
%& ArchitecturalStructure & 4 & 1 & (25.00\%) & & & 912 & (912)\\
%& Dam & 3 & 1 & (33.33\%) & & & 546 & (546)\\
%& RailwayLine & 2 & 2 & (100.00\%) & & & 7 & (7)\\
%& Zoo & 1 & 1 & (100.00\%) & & & 832 & (832)\\
%& Mountain & 1 & 1 & (100.00\%) & & & 1000 & (1000)\\
%& Island & 1 & 1 & (100.00\%) & & & 912 & (912)\\
%& Hospital & 1 & 1 & (100.00\%) & & & 1127 & (1127)\\
%& Airport & 1 & 1 & (100.00\%) & & & 1363 & (1363)\\
& (\# entities $< 15$) & 58 & 44 & (75.86\%) & & & 868 & (956)\\
\midrule
& Sub Total & 223 & 179 & (80.27\%) & & & 600 & (394)\\
\midrule
\multicolumn{2}{l}{GROUP}&&&&\\	
& Company & 188 & 113 & (60.11\%) & & & 509 & (361)\\
& SoccerClub & 26 & 13 & (50.00\%) & & & 780 & (741)\\
%& Organisation & 16 & 14 & (87.50\%) & & & 725 & (511)\\
%& PoliticalParty & 10 & 8 & (80.00\%) & & & 622 & (527)\\
& (\# entities $< 15$) & 10 & 8 & (80.00\%) & & & 687 & (526)\\
\midrule
& Sub Total & 240 & 148 & (61.67\%) & & & 559 & (412)\\
\midrule
\multicolumn{2}{l}{OTHER}&&&&\\	
& Species & 53 & 14 & (26.42\%) & & & 825 & (1008)\\
%& CelestialBody & 3 & 1 & (33.33\%) & & & 2 & (2)\\
%& Train & 2 & 2 & (100.00\%) & & & 241 & (241)\\
%& Aircraft & 1 & 1 & (100.00\%) & & & 1613 & (1613)\\
& (\# entities $< 15$) & 6 & 4 & (66.67\%) & & & 524 & (240)\\
\midrule
& Sub Total & 59 & 18 & (30.51\%) & &  & 758 & (977)\\
\midrule
\multicolumn{2}{l}{UNMAPPED} & 4891 & 3523 & (72.03\%) & & & 697 & (622)\\
\midrule
\multicolumn{2}{l}{\textbf{Total}}    & 13386 & 10762 & (80.40\%) & & & 578 & (417)\\
\bottomrule
        \end{tabular}

    \label{table:recdetail}
\end{table}


\begin{table}[!t]
\scriptsize
    \centering

        \begin{tabular}{lrrrr}
            \toprule
            \multicolumn{1}{l}{} & \multicolumn{2}{c}{\textbf{$\in$ Wikipedia}} & \multicolumn{1}{r}{\textbf{$\notin$ Wikipedia}} & \multicolumn{1}{r}{} \\
            \multicolumn{1}{c}{\textbf{daily tweets}} & \multicolumn{1}{r}{\textbf{\# uniq.}} & \multicolumn{1}{r}{\textbf{\# ambig.}} & \multicolumn{1}{r}{\textbf{}} & \multicolumn{1}{r}{\textbf{Total}} \\
            \midrule
			Mar.~21st, 2017       & 41 & 83 & 295 & 419\\
			Jun.~14th, 2017       & 35 & 77 & 283 & 395\\            
			Sep.~1st, 2017       & 41 & 66 & 327 & 434\\
        % \midrule
		%	\textbf{Total}        & 104 & 55 & 386 & 545\\
			\bottomrule
        \end{tabular}
        \caption{Details of the emerging entities discovered from the daily tweets with \textbf{Proposed (LSTM-CRF)}.}\label{table:precdetail}
\end{table}


\begin{table*}[!t]
\footnotesize
    \centering
        \begin{tabular}{llrrl@{\,}l}
            \toprule
            \textbf{TYPE} & \textbf{DBpedia types} & \textbf{\# entities} & \textbf{\# posts} & \multicolumn{2}{l}{\textbf{examples of emerging context (translated)}}\\ 
            \midrule
\textsc{\textsc{Person}}
& Actor & 885 & 2863 & * & Expected new voice actor ``\textbf{Sora Amamiya}'' appeared for \\ 
& MusicalArtist & 731 & 4616 & & the first time on  live broadcasting! It is becoming a topic...\\
& SoccerPlayer & 531 & 2327 & * & I saw ``Saints -End of Promise-'' at the new theater in  \\
& VoiceActor & 484 & 1596 & & Yokohama. It is a debut work of director \textbf{David Rowley} !!\\
& BaseballPlayer & 419 & 4390 & * & Ms. \textbf{Daruma Matsuura}, who won the newcomer award \\
& AdultActor & 299 & 1731 & & seems to start serializing from the next number.  \\
& Model & 281 & 1343 & * & Nice to meet you, I am \textbf{Tamotsu Kansyuji} from the\\
& Politician & 260 & 1164 & & Juno-Super-Boy Contest. From now  on I will try my best.\\
& Person & 177 & 729 & * & In Kawasaki Mayor's election, Mr. \textbf{Norihiko Fukuda} \\
& Writer & 152 & 542 & & defeated other candidates and was elected for the first time\\
& Wrestler & 136 & 576 & * & Mika, who is the partner of me has changed her name from \\ 
%& ComicsCreator & 93 & 361 & & Mika Tabura to \textbf{Momo Nonotomiya}\\
%& Presenter & 80 & 370 & * & Defeat 19th place in the world in the tour debut game! The world is paying \\
%& FigureSkater & 74 & 165 & &  attention to \textbf{Naomi Osaka}.\\
%& AthleticsPlayer & 68 & 296 & * & Yokohama DeNA Baystars announces that it has agreed to sign a player  contract for\\
%& BasketballPlayer & 66 & 175 & &  the 2017 season with \textbf{Spencer Patton}. \\
%& Military\textsc{Person} & 48 & 110 & * & I saw ``Saints - End of Promise -'' at the New Theater in Yokohama. It is a debut  \\
%& Comedian & 36 & 182 & & work of  featured director \textbf{David Rowley} !!! \\
%& Comedy\textsc{Group} & 28 & 82 & * & Mika, who is the partner of me has changed her name from ``Mika Tabura'' to \\
%& VolleyballPlayer & 21 & 70 & & ``\textbf{Momo Nonotomiya}''.  \\
%& Scientist & 19 & 94 & * & Nice to meet you, I am \textbf{Tamotsu Kansyuji} from the Juno-Super-Boy Contest. \\
%& TennisPlayer & 15 & 67 & & From now  on I will try my best as an actor. Thank you.  \\
%& Artist & 14 & 43\\
%& Philosopher & 4 & 5\\
%& Royalty & 3 & 7\\
%& Photographer & 3 & 4\\
%& FictionalCharacter & 3 & 19\\
%& MartialArtist & 1 & 6\\
%& Architect & 1 & 6\\
& (\# entities $< 100$, 17 types) & 577 & 2062 && Mika Tadokoro to \textbf{Mika Nonomiya} \\
\midrule
%& Sub Total & 4932 & 23939\\
%\midrule
\textsc{\textsc{Creative}}
& MusicSingle & 1321 & 11685 & * & Marvel \& Sony officially announced that the title of the \\
\textsc{\textsc{Work}}
& TelevisionShow & 1153 & 8478 & & rebooted version Spider-Man``\textbf{Spider-Man: Homecoming}''. \\
& MusicAlbum & 970 & 6092 & * & Congratulations on \textbf{Re: Zero-Starting Life in Another}\\
& Film & 917 & 6307 && \textbf{World} for upcoming publication! \\
& VideoGame & 652 & 6355 &*& KADOKAWA and Hatena's novel posting site \textbf{Kakuyomu} \\
& Manga & 623 & 2561 && will open on February 29,  2016. Web novel contest will be...\\
& Anime & 323 & 2983 &*& [Digest News] Asratec enters the robot software business\\
& RadioProgram & 266 & 1010 &&  with control software called ``\textbf{V-Sido OS}'' \\
& Book & 146 & 983 &*& It was announced on Shonen Jump released today,\\
& Song & 32 & 174 && new series ``\textbf{My Hero Accademia}'' starts from next week! \\
& Software & 28 & 360 &*& Give us a message at reply as we will record the first  \\
%& Website & 23 & 188 &&broadcast \textbf{Sasara Night of Fujioka Minami} on the STV.\\
%& Artwork & 4 & 12\\
%& ProgrammingLanguage & 2 & 79\\
& (\# entities $< 5$, 3 types) & 29 & 279 && broadcast \textbf{Sasara Night of Fujioka Minami} on the STV.\\
\midrule
%& Sub Total & 6460 & 47267 \\
%\midrule
\textsc{\textsc{Location}}
& Building & 121 & 756 &*&  As the result of voting, the name of the station to be built at\\
& Museum & 42 & 184 && the JR Nambu branch line is decided as \textbf{Odaei Station}!\\
& Station & 34 & 115 &*& A new gourmet building ``\textbf{Ueno no Mori Cherry Terrace}''\\
& Settlement & 28 & 47 &&  is born in Ueno. Both lunch and dinner can be eaten there. \\
& School & 24 & 34 &*& \textbf{Kumagai Morikazu Tsukechi Museum of Art} opening \\
& City & 17 & 46 && ceremony commenced. Director Konan's greetings are...\\
& University & 14 & 47 &*& Ekran, the popular station building of JR Kofu Station, which \\
& Mountain & 14 & 44 && was reborn as ``\textbf{CELEO Kohu}'' on the 13th.\\
%& Park & 11 & 30 \\
% & Temple & 9 & 52\\
% & Hospital & 8 & 18\\
% & Shrine & 7 & 18\\
% & Library & 7 & 31\\
% & RailwayLine & 6 & 64\\
% & Zoo & 4 & 8\\
% & WorldHeritageSite & 4 & 5\\
% & River & 4 & 10\\
%& Road & 3 & 9\\
%& Infrastructure & 2 & 5\\
%& ArchitecturalStructure & 2 & 7\\
%& SkiArea & 2 & 4\\
%& Dam & 3 & 10\\
%& Island & 2 & 3\\
%& Airport & 2 & 4\\
%& HotSpring & 1 & 3\\
& (\# entities $< 10$, 17 types) & 77 & 281 && \\
\midrule
%& Sub Total & 371 & 1554 \\
%\midrule
\textsc{\textsc{Group}}
& Company & 259 & 1441 &*& Mr. Ishiba decided on Friday to set up a political faction \\
& SoccerClub & 55 & 304 && and name it ``\textbf{Suigetsukai}.''\\
& Organization & 28 & 179 &*&  With the entry of robot business, Softbank established \\
& PoliticalParty & 24 & 249 && the new company named \textbf{Cocoro}\\
%& (\# entities $< 25$) & 24 & 249 \\
\midrule
%& Sub Total & 311 & 1869 \\
%\midrule
\textsc{Other}
& Species & 77 & 337 &*& New species \textbf{Sado flog}, found on Sado Island, features \\
& CelestialBody & 17 & 75 && yellow feet and yellow belly.\\
%& Thing & 14 & 102\\
% & MilitaryConflict & 7 & 9\\
% & ChemicalCompound & 7 & 16\\
% & Food & 1 & 2\\
% & Disease & 1 & 8\\
% & Aircraft & 1 & 5\\
% & Train & 2 & 4\\
% & Language & 3 & 3\\
& (\# entities $< 15$, 8 types) & 36 & 149 && \\

%\midrule
%& Sub Total & 116 & 459 \\
\midrule
\textsc{Unmapped} && 7345 & 35552 &*& JMA named the recent heavy rain as ``\textbf{Heavy Rainfall in  }\\
&&&&& / \textbf{Kanto Tohoku H27.9}''.\\
         \midrule
			\textbf{Total} && 19604 & 111046\\
			\bottomrule
			
        \end{tabular}
\caption{Statistics of the emerging entities and their contexts 
obtained from our Twitter archive by our time-sensitive distant supervision.}\label{table:ds}
\end{table*}
